Validity and Reliability of the Scale Internet Users' Information Privacy Concern (IUIPC) [Extended Version]

Internet Users' Information Privacy Concerns (IUIPC-10) is one of the most endorsed privacy concern scales. It is widely used in the evaluation of human factors of PETs and the investigation of the privacy paradox. Even though its predecessor Concern For Information Privacy (CFIP) has been evaluated independently and the instrument itself seen some scrutiny, we are still missing a dedicated confirmation of IUIPC-10, itself. We aim at closing this gap by systematically analyzing IUIPC's construct validity and reliability. We obtained three mutually independent samples with a total of $N = 1031$ participants. We conducted a confirmatory factor analysis (CFA) on our main sample. Having found weaknesses, we established further factor analyses to assert the dimensionality of IUIPC-10. We proposed a respecified instrument IUIPC-8 with improved psychometric properties. Finally, we validated our findings on a validation sample. While we could confirm the overall three-dimensionality of IUIPC-10, we found that IUIPC-10 consistently failed construct validity and reliability evaluations, calling into question the unidimensionality of its sub-scales Awareness and Control. Our respecified scale IUIPC-8 offers a statistically significantly better model and outperforms IUIPC-10's construct validity and reliability. The disconfirming evidence on the construct validity raises doubts how well IUIPC-10 measures the latent variable information privacy concern. The sub-par reliability could yield spurious and erratic results as well as attenuate relations with other latent variables, such as behavior. Thereby, the instrument could confound studies of human factors of PETs or the privacy paradox, in general.

==> IUIPC_FA-concordance.tex <==
\Sconcordance{concordance:IUIPC_FA.tex:IUIPC_FA.Rnw:%
1 21 1 50 0 1 5 529 1 2502 0}


==> IUIPC_FA_Child-concordance.tex <==
\Sconcordance{concordance:IUIPC_FA_Child.tex:IUIPC_FA_Child.Rnw:%
1 3 1 183 0 5 1 2 0 7 1 16 0 2 %
1 1679 0 713 1 3 0}


==> IUIPC_FA_ChildFAStats-concordance.tex <==
\Sconcordance{concordance:IUIPC_FA_ChildFAStats.tex:IUIPC_FA_ChildFAStats.Rnw:%
1 3 1 185 0 4 1 3 0 2 1 1 6 3 %
1 1 138 5 1 1 47 16 1 1 140 36 %
1 1 50 1 1 1 29 61 1 94 0 57 1 %
1 234 36 1 1 129 16 1 1 18 8 1 %
17 0 4 1 1 6 44 1 1 54 4 1 1 %
55 2 1 1 121 12 1 1 76 59 1 1 %
74 1 1 1 6 5 1 1 47 1 1 3 0}


==> corConvDiscrB.tex <==
\newcommand{\ccrtableB}{
% latex table generated in R 3.6.2 by xtable 1.8-4 package
% Tue May 12 13:30:21 2020
\begin{table*}[ht]
\centering
\caption{Convergent and discriminative validity for IUIPC-10 on Sample \textsf{B}} 
\label{tab:ccrtableB}
\begingroup\footnotesize
\begin{tabular}{rrllllllllll}
  \toprule
& & \multicolumn{3}{c}{Control} & \multicolumn{3}{c}{Awareness} & \multicolumn{4}{c}{Collection}\\
 \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-12}
& & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\ 
  \midrule
\multirow{3}{*}{Control} &  1. ctrl1 & --- &  &  &  &  &  &  &  &  &  \\ 
&  2. ctrl2 & \cellcolor{blue!25}0.55 & --- &  &  &  &  &  &  &  &  \\ 
 & 3. ctrl3 & \cellcolor{blue!25}0.27 & \cellcolor{blue!25}0.27 & --- &  &  &  &  &  &  &  \\ 
\multirow{3}{*}{Awareness} & 4. awa1 & 0.25 & 0.22 & 0.26 & --- &  &  &  &  &  &  \\ 
 & 5. awa2 & 0.31 & 0.3 & 0.3 & \cellcolor{blue!25}0.62 & --- &  &  &  &  &  \\ 
  &6. awa3 & 0.23 & 0.2 & 0.28 & \cellcolor{blue!25}0.32 & \cellcolor{blue!25}0.33 & --- &  &  &  &  \\ 
\multirow{4}{*}{Collection} & 7. coll1 & 0.06 & 0.06 & 0.28 & 0.05 & 0.11 & 0.33 & --- &  &  &  \\ 
&  8. coll2 & 0.11 & 0.07 & 0.3 & 0.22 & 0.24 & 0.31 & \cellcolor{blue!25}0.66 & --- &  &  \\ 
 & 9. coll3 & 0.16 & 0.09 & 0.32 & 0.17 & 0.22 & 0.4 & \cellcolor{blue!25}0.75 & \cellcolor{blue!25}0.71 & --- &  \\ 
 & 10. coll4 & 0.2 & 0.1 & 0.31 & 0.23 & 0.23 & 0.46 & \cellcolor{blue!25}0.7 & \cellcolor{blue!25}0.61 & \cellcolor{blue!25}0.81 & --- \\ 
   \bottomrule
\end{tabular}
 \\\emph{Note:} The marked cells close to the diagonal are correlations between items of the same constructs; they should be high for convergent validity. The unmarked cells away from the diagonal are correlations between non-construct items and the construct items; they should be low for discriminative validity.
\endgroup
\end{table*}
}

\newcommand{\ccrtableBcolorless}{
% latex table generated in R 3.6.2 by xtable 1.8-4 package
% Tue May 12 13:30:21 2020
\begin{table*}[ht]
\centering
\caption{Convergent and discriminative validity for IUIPC-10 on Sample \textsf{B}} 
\label{tab:ccrtableBcolorless}
\begingroup\footnotesize
\begin{tabular}{rrllllllllll}
  \toprule
& & \multicolumn{3}{c}{Control} & \multicolumn{3}{c}{Awareness} & \multicolumn{4}{c}{Collection}\\
 \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-12}
& & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\ 
  \midrule
\multirow{3}{*}{Control} &  1. ctrl1 & --- &  &  &  &  &  &  &  &  &  \\ 
&  2. ctrl2 & \textbf{0.55} & --- &  &  &  &  &  &  &  &  \\ 
 & 3. ctrl3 & \textbf{0.27} & \textbf{0.27} & --- &  &  &  &  &  &  &  \\ 
\multirow{3}{*}{Awareness} & 4. awa1 & 0.25 & 0.22 & 0.26 & --- &  &  &  &  &  &  \\ 
 & 5. awa2 & 0.31 & 0.3 & 0.3 & \textbf{0.62} & --- &  &  &  &  &  \\ 
  &6. awa3 & 0.23 & 0.2 & 0.28 & \textbf{0.32} & \textbf{0.33} & --- &  &  &  &  \\ 
\multirow{4}{*}{Collection} & 7. coll1 & 0.06 & 0.06 & 0.28 & 0.05 & 0.11 & 0.33 & --- &  &  &  \\ 
&  8. coll2 & 0.11 & 0.07 & 0.3 & 0.22 & 0.24 & 0.31 & \textbf{0.66} & --- &  &  \\ 
 & 9. coll3 & 0.16 & 0.09 & 0.32 & 0.17 & 0.22 & 0.4 & \textbf{0.75} & \textbf{0.71} & --- &  \\ 
 & 10. coll4 & 0.2 & 0.1 & 0.31 & 0.23 & 0.23 & 0.46 & \textbf{0.70} & \textbf{0.61} & \textbf{0.81} & --- \\ 
   \bottomrule
\end{tabular}
 \\\emph{Note:} The marked bold cells close to the diagonal are correlations between items of the same constructs; they should be high for convergent validity. The unmarked cells away from the diagonal are correlations between non-construct items and the construct items; they should be low for discriminative validity.
\endgroup
\end{table*}
}

==> efaloadings.tex <==
\newcommand{\efaloadingsCombined}{
\begin{table*}[tbp]
\centering\caption{Factor loadings of \textsf{Oblimin}-transformed EFA on Samples~\textsf{A} and~\textsf{B}}
\captionsetup{position=top}
\label{tab:efaloadingsCombined}
\subfloat[EFA on Sample \textsf{A} ($N_\mathsf{A} = 208$)]{
\label{tab:efaloadingsCombinedA}
\centering% latex table generated in R 3.6.2 by xtable 1.8-4 package
% Fri May  8 17:11:40 2020
\begingroup\footnotesize
\begin{tabular}{rrrrr}
  \toprule
  & \multicolumn{3}{c}{Factors} & \multirow{2}{*}{Uniqueness}\\
  \cmidrule(lr){2-4}
 & Collection & Awareness & Control &  \\ 
  \midrule
ctrl1 &  & 0.44 & 0.40 & 0.57 \\ 
  ctrl2 &  & 0.69 & 0.24 & 0.41 \\ 
  ctrl3 &  & 0.54 &  & 0.68 \\ 
  awa1 &  & 0.67 &  & 0.52 \\ 
  awa2 &  & 0.58 &  & 0.64 \\ 
  awa3 & 0.24 &  & 0.53 & 0.61 \\ 
  coll1 & 0.85 &  &  & 0.31 \\ 
  coll2 & 0.67 &  &  & 0.53 \\ 
  coll3 & 0.86 &  &  & 0.22 \\ 
  coll4 & 0.67 &  &  & 0.47 \\ 
   \midrule
SS loadings & 2.43 & 1.81 & 0.57 &  \\ 
  Proportion Var & 0.24 & 0.18 & 0.06 &  \\ 
  Cumulative Var & 0.24 & 0.42 & 0.48 &  \\ 
   \bottomrule
\multicolumn{5}{c}{\emph{Note:} $\chi^2(18) = 38.881, p = .003$, Variance explained $R^2=.48$}\\
\end{tabular}
\endgroup
}~\subfloat[EFA on Sample \textsf{B} ($N_\mathsf{B} = 391$)]{%
\label{tab:efaloadingsCombinedB}
\centering% latex table generated in R 3.6.2 by xtable 1.8-4 package
% Fri May  8 17:11:40 2020
\begingroup\footnotesize
\begin{tabular}{rrrrr}
  \toprule
    & \multicolumn{3}{c}{Factors} & \multirow{2}{*}{Uniqueness}\\
  \cmidrule(lr){2-4}
 & Collection & Awareness & Control & \\ 
  \midrule
ctrl1 &  &  & 0.70 & 0.48 \\ 
  ctrl2 &  &  & 0.78 & 0.42 \\ 
  ctrl3 & 0.27 &  & 0.26 & 0.76 \\ 
  awa1 &  & 0.88 &  & 0.26 \\ 
  awa2 &  & 0.66 &  & 0.45 \\ 
  awa3 & 0.36 & 0.25 &  & 0.70 \\ 
  coll1 & 0.86 &  &  & 0.31 \\ 
  coll2 & 0.74 &  &  & 0.42 \\ 
  coll3 & 0.93 &  &  & 0.14 \\ 
  coll4 & 0.84 &  &  & 0.25 \\ 
   \midrule
SS loadings & 3.07 & 1.33 & 1.21 &  \\ 
  Proportion Var & 0.31 & 0.13 & 0.12 &  \\ 
  Cumulative Var & 0.31 & 0.44 & 0.56 &  \\ 
   \bottomrule
\multicolumn{5}{c}{\emph{Note:} $\chi^2(18) = 39.918, p = .002$, Variance explained $R^2=.56$}\\
\end{tabular}
\endgroup
}
\end{table*}
}

